Formal Modelling of a Usable Identity Management Solution for Virtual Organisations

This paper attempts to accurately model security requirements for computational grid environments with particular focus on authentication. We introduce the Audited Credential Delegation (ACD) architecture as a solution to some of the virtual organisations identity management usability problems. The approach uses two complementary models: one is state based, described in Z notation, and the other is event-based, expressed in the Process Algebra of Hoare's Communicating Sequential Processes (CSP). The former will be used to capture the state of the WS and to model back-end operations on it whereas the latter will be used to model behavior, and in particular, front-end interactions and communications. The modelling helps to clearly and precisely understand functional and security requirements and provide a basis for verifying that the system meets its intended requirements.

==> eptcsdata.tex <==
\providecommand{\event}{Jeremy W. Bryans and John S. Fitzgerald (Eds.): \\
Formal Aspects of Virtual Organisations 2009 (FAVO2009)}
\providecommand{\volume}{16}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{41}
\providecommand{\eid}{4}

